Ensemble-based Blackbox Attacks on Dense Prediction

We propose an approach for adversarial attacks on dense prediction models (such as object detectors and segmentation). It is well known that the attacks generated by a single surrogate model do not transfer to arbitrary (blackbox) victim models. Furthermore, targeted attacks are often more challenging than the untargeted attacks. In this paper, we show that a carefully designed ensemble can create effective attacks for a number of victim models. In particular, we show that normalization of the weights for individual models plays a critical role in the success of the attacks. We then demonstrate that by adjusting the weights of the ensemble according to the victim model can further improve the performance of the attacks. We performed a number of experiments for object detectors and segmentation to highlight the significance of the our proposed methods. Our proposed ensemble-based method outperforms existing blackbox attack methods for object detection and segmentation. Finally we show that our proposed method can also generate a single perturbation that can fool multiple blackbox detection and segmentation models simultaneously. Code is available at https://github.com/CSIPlab/EBAD.

==> tables/tab-rebuttal-obj-compare-conventional.tex <==
\begin{wraptable}{r}{3.2cm}
\vspace{-5mm}
\hspace{-7mm}
\centering
\footnotesize
\begin{tabular}{lcc}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ATSS} \\
 & mAP $\downarrow$ & $Q$ $\downarrow$ \\ \hline
Clean & 0.54 & N/A \\
PRFA & 0.20 & 3500 \\
\text{[27]} & 0.04 & 1837 \\
Ours & \textbf{0.00} & \textbf{10} \\ \hline
\end{tabular}
\vspace{-5mm}
\end{wraptable}


==> tables/tab-rebuttal-obj-different-surrogates.tex <==
\begin{table}[h]
\vspace{-7mm}
\centering
\caption{Replacing YOLOv3 with Def. DETR} \label{tab:obj-replaceYOLO}
\footnotesize
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{WB~/~WO} & \multicolumn{2}{c}{\textbf{Surrogate}} & \multicolumn{5}{c}{\textbf{Blackbox Victims}} \\
 & FRCNN & Def. & Ret. & Lib. & Fov. & Free & DETR \\ \hline
\xmark ~/ \xmark & 8.5 & 69.5 & 10.6 & 4.0 & 8.0 & 10.5 & 12.0 \\
\xmark ~/ \cmark & 34.6 & 94.3 & 36.7 & 25.0 & 33.5 & 53.0 & 38.5 \\
\cmark ~/ \xmark & 68.0 & 80.5 & 47.2 & 38.5 & 37.5 & 57.5 & 26.5 \\
\cmark ~/ \cmark & \textbf{88.1} & \textbf{95.0} & \textbf{74.9} & \textbf{70.5} & \textbf{73.0} & \textbf{84.0} & \textbf{56.0} \\
\text{ZQA} & 88.2 & - & 44.0 & 51.4 & 53.4 & - & - \\
\hline
\end{tabular}
\vspace{-3.5mm}
\end{table}
